The Nun Path: The Evolution and Quenching of Satellite Galaxies

The galaxy quenching process, in which a galaxy stops forming stars is a crucial stage in galaxy life. Two mechanisms for quenching are possible: halo mass quenching of central galaxies and environmental quenching of satellite galaxies. This thesis describes the satellite galaxies (SG) quenching process and its primary causes. The analysis contains a study of a large sample of 118 SGs within the Vela cosmological simulation, identified by a specific SG merger tree algorithm. We find that the quenching evolves through a typical path in the diagram of specific star formation (sSFR) vs. inner stellar surface density ($\Sigma_{\star, 0.5\textrm kpc}$), with the inner surface density defined as the density within 0.5kpc from the center of mass of the SG. Three discrete phases characterize this path: 1. Halt in gas accretion with SG compaction at high sSFR as the SG keeps forming stars 2. Gas removal and rapid drop in the sSFR at the peri-center of its orbit within the host halo 3. Stellar heating and stripping may lead to coalescing with the halo center, an ultra-diffuse galaxy (UDG), a compact elliptical galaxy (eCg), or a globular cluster (GC). We find that the main drivers of SG evolution are ram pressure stripping at the initial stages and tidal forces at the final stages, aided by starvation, suppression of gas accretion. We show that other processes, such as gas depletion by star formation or stellar feedback are secondary. Moreover, we present an innovative method for constructing merger trees in simulations that solve systemic errors. Two new significant results presented here: a. Decoupling of dark-matter from the stellar component in SGs. b. Compact elliptical SG formation. An assembly of these results and others are presented in a fast and robust catalog.

==> chapters/appendices/app0A.tex <==
%
% file: app0A.tex
% author: Tomer Nussbaum
% description: ?
%
% 
\chapter{Elliptical galaxy formation (eCg) }
\label{app:app01}

\initial{W}e present here \textbf{preliminary} additional visualizations regarding SG 22-004, the eCg case.

The galaxy was formed in a filament, the full filament is hard to observe via 2d picture. Therefore we supply a 3D interactive model of the filament. Available here: 
\textcolor{blue}{\href{https://skfb.ly/6wxpS}{Filament Model}} When the surfaces are iso-densities contours of the filament. Fig~\ref{fig:Formation_in_filament} presents the first identification snapshot and Fig~\ref{fig:eCg_example} present the SG evolution product, an eCg.

Also we provide here five \textbf{preliminary} 3D-models representing different stages in the SG 22-004 evolution: 
\cite{Kiyun2019} jellyfish

1. Entering Rvir
2. Contraction & sSFR decrease - https://skfb.ly/6wwnn
3. Mid sSFR - https://skfb.ly/6wwnn
4. No sSFR - https://skfb.ly/6wwus
5. Sigma 0.5kpc fall


\begin{figure}[H] \centering
\includegraphics[width=0.9\linewidth]{chapters/appendices/fig0A/2204_FormationA.jpeg}
\includegraphics[width=0.9\linewidth]{chapters/appendices/fig0A/2204_FormationB.jpeg}	\caption{\small \textbf{Formation in a filament, gas rich environment} 
The figure is divided to 4 plots, each of them shows a different projected mass quantity. from left to right, up then down: stars, gas, dark matter and total mass. colored is the summed mass in a cell. Note that each subplot is divided to three subsubplots, they represent different projections, y-x,y-z,x-z, in order to grasp the 3d shape of the galaxy. The circle represent the approximated $R_{\textrm sat}$.
\hspace{0.5} The figure shows the eCg first identification snapshot at the VELA simulation before it was. we can see the formation moment of the SG in a very high dense gas region inside a filament. }
 \label{fig:Formation_in_filament}
\end{figure}

\begin{figure}[H] \centering
\includegraphics[width=0.9\linewidth]{chapters/appendices/fig0A/2204_eCgA.jpeg}
\includegraphics[width=0.9\linewidth]{chapters/appendices/fig0A/2204_eCgB.jpeg}
\caption{\small \textbf{eCg example} 
Colors and methods are similar to Fig.~\ref{fig:fig:Formation_in_filament}
\hspace{0.5} In this figure we can see a clear elliptical compact galaxy without gas or dark matter}
\label{fig:eCg_example}
\end{figure}

\textcolor{red}{3D model}
filament, 1,2,3,4,5





% \textcolor{red}{Maybe add UDG which losses all its dark matter}
